Confronting Ambiguity in 6D Object Pose Estimation via Score-Based Diffusion on SE(3)

Addressing pose ambiguity in 6D object pose estimation from single RGB images presents a significant challenge, particularly due to object symmetries or occlusions. In response, we introduce a novel score-based diffusion method applied to the $SE(3)$ group, marking the first application of diffusion models to $SE(3)$ within the image domain, specifically tailored for pose estimation tasks. Extensive evaluations demonstrate the method's efficacy in handling pose ambiguity, mitigating perspective-induced ambiguity, and showcasing the robustness of our surrogate Stein score formulation on $SE(3)$. This formulation not only improves the convergence of denoising process but also enhances computational efficiency. Thus, we pioneer a promising strategy for 6D object pose estimation.

==> sec/D_future.tex <==


\section{Limitations and Broader Impacts}
\label{sec:limitation}

While our score model on $SE(3)$ performs well on the synthetic datasets, there are still limitations in real-world applications. In the SYMSOL experiment, we observed that training a single score model across multiple shapes can be affected by the interactions between the distributions of different objects. This interaction leads to a slight decrease in performance and poses a challenge when extending the model to real-world datasets~\cite{hodavn2020bop} featuring a wide variety of objects and occlusions.

From an architectural perspective, the current design, which conditions image feature embeddings represented by low-dimensional vector values on the score model, can potentially create a bottleneck due to the limited amount of information it can carry. Therefore, future work could explore better architectures. This might involve integrating high-dimensional image features with the score model or devising improved methods for learning image feature representations. These improvements could allow our score models to be applied in more complex scenarios in the future research endeavors.
